Faster Deterministic All Pairs Shortest Paths in Congest Model

We present a new deterministic algorithm for distributed weighted all pairs shortest paths (APSP) in both undirected and directed graphs. Our algorithm runs in $\tilde{O}(n^{4/3})$ rounds in the Congest models on graphs with arbitrary edge weights, and it improves on the previous $\tilde{O}(n^{3/2})$ bound of Agarwal et al. [ARKP18]. The main components of our new algorithm are a new faster technique for constructing blocker set deterministically and a new pipelined method for deterministically propagating distance values from source nodes to the blocker set nodes in the network. Both of these techniques have potential applications to other distributed algorithms. Our new deterministic algorithm for computing blocker set adapts the NC approximate hypergraph set cover algorithm in [BRS94] to the distributed construction of a blocker set. It follows the two-step process of first designing a randomized algorithm that uses only pairwise independence, and then derandomizes this algorithm using a sample space of linear size. This algorithm runs in almost the same number of rounds as the initial step in our APSP algorithm that computes $h$-hops shortest paths, and significantly improves on the deterministic blocker set algorithms in [ARKP18, AR19] by removing an additional $n\cdot |Q|$ term in the round bound, where Q is the blocker set. The other new component in our APSP algorithm is a deterministic pipelined approach to propagate distance values from source nodes to blocker nodes. We use a simple natural round-robin method for this step, and we show using a suitable progress measure that it achieve the $\tilde{O}(n^{4/3})$ bound on the number of rounds. It appears that the standard deterministic methods for efficiently broadcasting multiple values, and for sending or receiving messages using the routing schedule in [HPDG+19,LSP19] do not apply to this setting.

==> overview.tex <==
\vspace{-.15in}
\section{Overview of Techniques}	\label{sec:overview}

\vspace{-.05in}

Our APSP algorithm is based on two important techniques: a faster deterministic construction of the blocker set, and a faster method to send distance values $\delta (x,c)$ to blocker nodes $c$.

\vspace{-.2in}
\subparagraph*{Blocker Set.}
The previous best bound for computing blocker set deterministically is due to~\cite{ARKP18, AR19}. 
The issue with the bounds in~\cite{ARKP18, AR19} is that there is an additional $n\cdot |Q|$ term, where $Q$ is the blocker set, in the round bound (recall $|Q| = \Theta(\frac{n\log n}{h})$),
making these algorithms only suitable for constructing smaller-sized blocker sets.
In this paper we address this by getting rid of this term in the round complexity.

In Section~\ref{sec:blocker} we present a randomized algorithm for constructing blocker set, using ideas from the 
RNC Set Cover algorithm of Berger et al.~\cite{BRS94}. 
We then use an exhaustive search technique of Luby~\cite{Luby93} to obtain a deterministic blocker set algorithm 
(Section~\ref{sec:deterministic-blocker}).
Given an arbitrary source set $S$,
our deterministic algorithm for computing blocker set takes $\tilde{O}(|S|\cdot h)$ rounds, which is only a polylogarithmic factor away from the bound for constructing initial $h$ hop CSSSP.

\vspace{-.2in}
\subparagraph*{Communicate distance values $\delta (x,c)$ to blocker nodes $c$.}
A trivial way to implement this is to broadcast all distance values in the network.
This takes $O(n\cdot |Q|)$ rounds and is the current best bound for implementing this step deterministically.
In Section~\ref{sec:frames} we describe a distributed algorithm to implement this step in $\tilde{O}(n\cdot \sqrt{|Q|})$
rounds.
Our algorithm uses a simple round-robin pipelined approach, however its proof of correctness is quite subtle.  

The first step in our algorithm is to reduce the congestion to at most $n\cdot \sqrt{|Q|}$ using a technique similar to a randomized 
algorithm in~\cite{HNS17}.
One solution to send these distance values is to allow every node to send an unsent message to its parent in the corresponding tree.
However this approach may cause some nodes to keep waiting for messages to arrive for some blocker nodes $c$. 
This can happen if the child nodes are busy sending out messages for other blocker nodes.
Thus this approach, in the worst case, may need $O(n\cdot |Q|)$ rounds in total.
Another solution is to dedicate a single round globally to a particular blocker node $c$.
However this approach may also require $n\cdot |Q|$ rounds in the worst case, since there can be $\Theta(n)$ different messages for $c$ and thus require $\Theta(n)$ rounds for them  to reach $c$.

We solve these issues  by just using a simple round-robin approach and we introduce a new notion of \textit{frames}, to establish that 
this approach works.
The advantage of using frames is that on the one hand, it ensures that every node receives a message for every blocker node $c$ in every
frame, thus eliminating the issue of endless waiting for messages to arrive for a particular blocker node $c$.
Another advantage is that it eliminates the need to assign a global round to any blocker node $c$, thus reducing the overall round 
complexity.


==> related.tex <==
%\vspace{-.15in}

\subsection{Related Work}	\label{sec:related}
	
%\vspace{-.05in}

The current best bound for the weighted APSP problem is the randomized algorithm of Bernstein and Nanongkai~\cite{BN19} that runs in 
$\tilde{O}(n)$ rounds. 
This result works for arbitrary edge weighted graphs and holds with w.h.p. in $n$.
For the deterministic case, the APSP algorithm of Agarwal et al.~\cite{ARKP18} that runs in $\tilde{O}(n^{3/2})$ rounds is the best 
bound for arbitrary edge weighted graphs.
However for graphs with integer edge weights, the recent result of Agarwal and Ramachandran~\cite{AR19} improves on this bound when 
the edge weights are bounded by $n^{1\epsilon}$ or shortest path distances bounded by $n^{3/2-\epsilon}$.
There is a $\Omega (n)$ lower bound for this problem~\cite{CKP17}, which holds even for the unweighted case, but it is not deterministic.

In this paper we present a deterministic algorithm for arbitrary edge weighted graphs that runs in 
$\tilde{O}(n^{4/3})$ rounds, improving on the $\tilde{O}(n^{3/2})$ deterministic APSP bound of Agarwal et al.~\cite{ARKP18}.

\textbf{Other Related Works.}
For graphs with positive integer edge weights, deterministic $\tilde{O}(n/\epsilon^2)$-round algorithms for obtaining a $(1+\epsilon)$ 
approximation to APSP are known~\cite{LP15,Nanongkai14}.
This was recently extended to also include zero edge weights in~\cite{AR19}, while matching the same $\tilde{O}(n/\epsilon^2)$-round
bound.
For unweighted graphs, several $O(n)$ round algorithms for computing APSP are known~\cite{LP13,HW12,PRT12}.
